Complexity Results on Register Pushdown Automata

Register pushdown automata (RPDA) is an extension of classical pushdown automata to handle data values in a restricted way. RPDA attracts attention as a model of a query language for structured documents with data values. The membership and emptiness problems for RPDA are known to be EXPTIME-complete. This paper shows the membership problem becomes PSPACE-complete and NP-complete for nondecreasing and growing RPDA, respectively, while the emptiness problem remains EXPTIME-complete for these subclasses.

==> acknowledgements.tex <==
\section*{Acknowledgements}
This work was supported by JSPS KAKENHI Grant Number\\
JP19H04083. 
